Detecting Social Influence in Event Cascades by Comparing Discriminative Rankers

The global dynamics of event cascades are often governed by the local dynamics of peer influence. However, detecting social influence from observational data is challenging due to confounds like homophily and practical issues like missing data. We propose a simple discriminative method to detect influence from observational data. The core of the approach is to train a ranking algorithm to predict the source of the next event in a cascade, and compare its out-of-sample accuracy against a competitive baseline which lacks access to features corresponding to social influence. We analyze synthetically generated data to show that this method correctly identifies influence in the presence of confounds, and is robust to both missing data and misspecification --- unlike well-known alternatives. We apply the method to two real-world datasets: (1) the co-sponsorship of legislation in the U.S. House of Representatives on a social network of shared campaign donors; (2) rumors about the Higgs boson discovery on a follower network of $10^5$ Twitter accounts. Our model identifies the role of social influence in these scenarios and uses it to make more accurate predictions about the future trajectory of cascades.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> generative.tex <==
\section{Data generation}
\label{sec:generative}
% motivation behind synthetic data generation
To demonstrate the relative effectiveness of our method in identifying social influence, we need data about the network connections and individual adoption actions of some behavior.
Although such data is becoming increasingly available from online activities in a social network, evaluating our method on real data suffers from three limitations. 
First, in real data the reason behind the spread -- whether it was caused by influence or by homophily -- is not always clearly established. 
Second, the extent of both homophily and influence is not known beforehand making it difficult to evaluate any method's robustness under different conditions.
And finally, any method should be evaluated against a number of instances under similar conditions to determine its true statistical strength.
Due to these limitations, we instead simulate the data synthetically using a stochastic generative model that is parameterized to control the effects of homophily and influence.
Synthetically generating the data eliminates all the aforementioned limitations: we can precisely control for all the competing causes and generate data under all these conditions repeatedly.

% explain the terminology throughout the paper
For consistency, we first describe some terminology that we use throughout the rest of the paper.
Any method that detects influence requires information about the network: who is connected to whom; and the sequence of adoptions by nodes for some behavior.
Such a sequence of adoption actions is called a cascade.
Every individual adoption action in the sequence is identified by a pair -- the adopter node and the time at which action was taken -- and is called an event.
For every event, the adopter is called as the source of that event. 
A node is said to be activated every time when it is the source of an event. 
The total number of events in the cascade is defined as the length of the cascade.


Our stochastic model can generate cascades of a given length under different conditions.
Specifically, the events in a cascade are generated using a multivariate Hawkes process (HP), which is a special kind of inhomogenous Poisson process such that the rate of generating the events is modulated by the history of events in the past~\citep{hawkes1971spectra}.
Like any Poisson process, the HP is described by its intensity function defined for every node in the network. \footnote{The intensity function of HP is called conditional intensity to indicate that it depends on the past}
The intensity function defines the instantaneous rate at which events are generated. 
The cascade is generated by drawing events from HP as follows.

\begin{align}
\forall n, (t_n, s_n) \sim {\Hawkes}\left(
     \begin{array}{c}
     \lambda_{1}\left(t\right)\\
	 \lambda_{2}\left(t\right)\\
	 \vdots\\
	 \lambda_{M}\left(t\right)
     \end{array}
\right),
\end{align}
where $t_n$ is the timestamp and $s_n$ is the source of the $n^{th}$ event.
In general, the intensity of HP for a single node $i$ is given as,
\begin{align}
\label{eq:mhp-cond-int}
\lambda_{i}\left(t\right) = \mu_{i} + \sum\limits_{j=1}^{M}\sum\limits_{\substack{\tau:\tau < t \\ \tau \in \Tcal_{j}}} \alpha_{\edge{j}{i}}\kernelband{\omega}{t-\tau},
\end{align}

$\mubf$, $\alphabf$ and $\omega$ are the parameters of the intensity function; $M$ is the total number of nodes in the network; and $\Tcal_{j}$ is the set of events whose source is $j$. 
$\mubf$ denotes the base rate at which nodes generate events, whereas $\alphabf$ is the pairwise influence between nodes in the network.
To generate cascades under conditions of social influence and other confounds, such as homophily, we make the following two parametric modifications to the intensity function. 
%The algorithm to generate the data using the hawkes process when the parameters are known is given in Appendix~\ref{sec:simulator}.
%Network cascades for different scenarios can be generated by tuning these parameters.
%For our generation process, we use the following parameter settings.

\begin{align}
\alpha_{\edge{j}{i}} &= 
\begin{cases}
\label{eq:influence-generative}
a & \text{if } j=i \\
b & \text{if } j \neq i \text{ and } \delta\left(A_{\edge{j}{i}}\right) \\ 
0 & \text{otherwise}
\end{cases} \\
\label{eq:homophily-generative}
\mu_i &= \sigma\left(\beta v_i^{(2)} + \eta\right)
\end{align}
where $v_i^{(2)}$ is the second eigen vector of the laplacian matrix of the network; $\sigma(\cdot)$ is the sigmoid function used to keep the base rate to be positive; and $A$ is the adjacency matrix of the network with $\delta(\cdot)$ being the dirac delta function.

Finally, our underlying networks are Twitter mention networks. 
The nodes in the network are users who used a partisan political hashtag during a specified period in the 2016 election cycle, whereas the edges are when a user mentions other user. The networks are directed and static.  
\todo{Need to expand the last paragraph about networks more. The first equation does not add more maybe I should remove that and instead explain more of how the different conditions can be achieved.}
